Single CASANOVA? Not in multiple comparisons

When comparing multiple groups in clinical trials, we are not only interested in whether there is a difference between any groups but rather the location. Such research questions lead to testing multiple individual hypotheses. To control the familywise error rate (FWER), we must apply some corrections or introduce tests that control the FWER by design. In the case of time-to-event data, a Bonferroni-corrected log-rank test is commonly used. This approach has two significant drawbacks: (i) it loses power when the proportional hazards assumption is violated [1] and (ii) the correction generally leads to a lower power, especially when the test statistics are not independent [2]. We propose two new tests based on combined weighted log-rank tests. One as a simple multiple contrast test of weighted log-rank tests and one as an extension of the so-called CASANOVA test [3]. The latter was introduced for factorial designs. We propose a new multiple contrast test based on the CASANOVA approach. Our test promises to be more powerful under crossing hazards and eliminates the need for additional p-value correction. We assess the performance of our tests through extensive Monte Carlo simulation studies covering both proportional and non-proportional hazard scenarios. Finally, we apply the new and reference methods to a real-world data example. The new approaches control the FWER and show reasonable power in all scenarios. They outperform the adjusted approaches in some non-proportional settings in terms of power.

==> archiv.tex <==
{\color{blue} 
Time-to-event analysis, also known as survival analysis, plays a crucial role in various fields such as medical research, engineering, and social sciences. Many trials comprise multiple groups (treatment arms) or even have a factorial structure, which poses unique statistical methodological challenges. The primary research question in such trials is manifold and rarely subject to whether \textit{any} of the arms differ from the others. Most of the times we are interested in the exact treatment groups that differ from each other. Therefore, global test procedures, such as quadratic forms (ANOVA-type methods) to test null hypotheses of equality of hazard ratios or cumulative hazard rate functions, cannot be used to answer the main question and are therefore often not the method of choice \cite{Konietschke2012, ditzhausCASANOVAPermutationInference2021}. On the contrary, flexible multiple comparison procedures that can be adapted to the question of interest and especially to factorial designs are key in modern data analysis.  Up until now, existing procedures use pairwise multiple log-rank tests and adjust for multiplicity with a certain correction (e.g., Bonferroni) \cite{logan2005pairwise}. They often lack efficiency, because they either do not take the correlation across the multiple test statistics into account or are subject to rather restrictive dependency assumptions, e.g., the joint distribution of the test statistics is of multivariate totally positive order two \cite{Gao2008,gao2008nonparametric}. In recent years, many researchers developed \textit{multiple contrast test procedures} (MCTPs) along with simultaneous confidence intervals (SCIs) (usually conducted as maximum tests), which are valid for arbitrary correlations of the test statistics and use the correlation within the multiplicity adjustment for various endpoints (means, proportions, Mann-Whitney effects) \cite{Bretz2001,schaarschmidt2009asymptotic,hasler2008multiple,konietschke2013multiple,blanche2022closed}. \cite{munko2024} introduced a restricted mean survival time (RMST)-based multiple contrast tests for time-to-event data. Since the RMST should not be employed under crossing hazards \cite{dormuth2022test, dormuth2023comparative}, we aim to close this gap and introduce a powerful and flexible MCTP for the analysis of survival data with crossing hazards.

In survival analysis, the log-rank test is one of the most prominent test procedures. It is well known that the method is optimal when the proportional hazards (PH) assumption is met but significantly loses power otherwise \cite{dormuth2023comparative}. Even though the problem is fairly well known, a substantial amount of investigators of (clinical) trials still ignore the issue and publish their findings upon log-rank tests in leading high-quality peer-review journals even when the assumption is violated \cite{kristiansen2012prm39,trinquart2016comparison, dormuth2023comparative}. For the analysis of two independent samples, weighted log-rank tests and their combinations comprise a great alternative to the classical log rank-test and are beneficial in non-proportional hazards models \cite{andersen2012statistical, fleming2013counting, BrendelETAL2014, DitzhausFriedrich2018}. The latter comprises multiple weight functions within a single multivariate test. Which weight function to choose depends on the alternative of interest and cannot be recommended in a general way. However, the test is a global Wald-type statistic (quadratic form), and if it rejects the null hypothesis at a respective significance level $\alpha \in (0,1)$, it does not provide the information on which weight function appears most powerful. For the analysis of more than two samples and factorial designs, Ditzhaus et al. extended these procedures to the \textit{Cumulative Aalen Survival Analysis-of-Variance} (CASANOVA) \cite{ditzhausCASANOVAPermutationInference2021} method. In principle, they are global ANOVA-based tests (quadratic forms) and can be used for estimating and testing main and interaction effects in general factorial designs. Estimation and testing of user-specific contrasts are not possible which limits its application in statistical practice. To overcome these shortcomings, we propose a novel flexible MCTP. Extensive simulation studies indicate that the test is more powerful under non-proportional hazards and eliminates the need for additional p-value correction. The remainder of the paper is organized as follows. In the second section, we introduce the main statistical methods employed in the analyses. We describe the simulation setup and the corresponding results in the third section. The methods of interest are applied to a real-world data example in the following section. The final conclusions are drawn in section five, together with future research questions.
}

\iffalse
In the context of time-to-event data, traditional global test procedures can provide valuable insights into the overall significance of treatment effects across groups. However, they fall short of providing specific information about which particular groups differ from one another in the event occurrence. In contrast, multiple contrast tests have emerged as an appealing alternative, offering a more comprehensive and informative approach to analyzing several-sample time-to-event data.

The primary objective of this paper is to address the challenges associated with time-to-event analysis in the several-sample case, with a specific focus on robustness in non-proportional hazards settings. Non-proportional hazards are common in survival data, where the hazard rates for different groups may vary over time, posing additional complexities for statistical inference. Our proposed multiple contrast tests aim to overcome these challenges and yield accurate results, even in the presence of non-proportional hazards.

One of the key advantages of multiple contrast tests is their ability to provide detailed information regarding group differences. When a significant outcome is observed, these tests not only reveal the presence of at least one differing group but also identify the specific groups that exhibit distinct event occurrence patterns. This level of granularity offers invaluable insights for researchers seeking to understand the impact of various treatments or interventions.

Moreover, our proposed multiple contrast tests leverage the correlation across the test statistics, making them particularly powerful in detecting treatment effects. By considering the relationships between multiple comparisons, these tests achieve enhanced statistical efficiency and sensitivity, thereby increasing the likelihood of correctly identifying true group differences.

Throughout this paper, we will introduce the statistical model and methodology behind our multiple contrast tests for time-to-event data. We will present point estimators of treatment effects and variances, along with detailed explanations of the multiple contrast test procedures. Additionally, we will discuss methods for estimating sample sizes, which are vital for conducting meaningful and adequately powered time-to-event studies.

In conclusion, this paper aims to provide a comprehensive and robust solution for analyzing time-to-event data in a several-sample setting. The proposed multiple contrast tests offer valuable insights into group differences, even in the presence of non-proportional hazards, and are poised to become an essential tool in survival analysis research.}
Time-to-event data pose specific challenges in hypothesis testing, and multiple testing plays a vital role in time-to-event analysis. {\color{blue} Up until now, traditional multiple testing methods, such as the Bonferroni or Bonferroni Holm correction, are used for multiplicity adjustment.} However, traditional multiple testing methods have primarily focused on continuous outcomes or binary responses in their development and application  \textcolor{red}{source}. In the context of survival analysis, the commonly used approach for multiple hypothesis testing has been the Bonferroni-adjusted log-rank test \textcolor{red}{source}. Nevertheless, it is well recognized that the Bonferroni method does not fully exploit the family-wise error rate. Furthermore, the assumption of proportional hazards, which is often violated in practice, hampers the effectiveness of the log-rank test, as it is optimal only under this assumption, leading to potential loss of power \textcolor{red}{source}.

To address these limitations, we propose a novel multiple-testing approach tailored specifically for non-proportional time-to-event data. 


In recent years, \Ina{Literaturübersicht}

The objective of this article is to introduce novel approaches that effectively control the family-wise error rate (FWER) and demonstrate robustness in non-proportional hazards settings. To achieve this, we integrate the concept of maximum tests with multidirectional log-rank tests. In the subsequent section, we present existing comparison methods, along with our proposed innovative approaches. The third section encompasses the simulation setup, where we outline the design and parameters employed and subsequently present the results obtained from applying the introduced methods. Additionally, we evaluate the performance of these approaches using a real-world dataset. Finally, a comprehensive discussion of all the results is provided, and practical recommendations are made to guide users in their application.
